Dynamic neighbourhood optimisation for task allocation using multi-agent

In large-scale systems there are fundamental challenges when centralised techniques are used for task allocation. The number of interactions is limited by resource constraints such as on computation, storage, and network communication. We can increase scalability by implementing the system as a distributed task-allocation system, sharing tasks across many agents. However, this also increases the resource cost of communications and synchronisation, and is difficult to scale. In this paper we present four algorithms to solve these problems. The combination of these algorithms enable each agent to improve their task allocation strategy through reinforcement learning, while changing how much they explore the system in response to how optimal they believe their current strategy is, given their past experience. We focus on distributed agent systems where the agents' behaviours are constrained by resource usage limits, limiting agents to local rather than system-wide knowledge. We evaluate these algorithms in a simulated environment where agents are given a task composed of multiple subtasks that must be allocated to other agents with differing capabilities, to then carry out those tasks. We also simulate real-life system effects such as networking instability. Our solution is shown to solve the task allocation problem to 6.7% of the theoretical optimal within the system configurations considered. It provides 5x better performance recovery over no-knowledge retention approaches when system connectivity is impacted, and is tested against systems up to 100 agents with less than a 9% impact on the algorithms' performance.

==> problem-allocation-implications.tex <==
\subsubsection{Implications of capabilities and resource pressure}
\reviewquestionopen{
	what is the use of section 3.3.3 ? These properties do not bring much to the paper. The third one is hard to be convinced of without a proper demonstration, especially since if I understand eq(5) as "within the SYSTEM", what happens if on* is NOT on the current pairwise distinct neighbourhood of the system ?
}

The different agent capabilities mean that there are a limited number of agents that can complete a given atomic task type, increasing the resource pressure effect on the quality of atomic tasks. Given this, there exists system-wide competition between parent agents for child agents' resources that can change individual optimal allocation solutions compared to where there is no competition.

\begin{property}[Allocation state]
	An agent $\varAgent{}{}$  is allocated a composite task $\varCompositeTask{}{}$ composed of a set of atomic tasks. If the agent has a set of neighbours $\functionNeighbourhoodSignature{}{}$ then one of the following will be true,
	\begin{enumerate}{
			\item For each atomic task in the composite task, the capability required to complete the task is provided by one of the agents in the neighbourhood, $\exists \tupleAgent{}{} \in \functionNeighbourhoodSignature{}{}$.
			The composite task can be successfully allocated to $\varAgent{}{}$ and completed. A locally optimal allocation exists.
			
			\item The capabilities required for the atomic tasks composing the composite task cannot be provided by agents within the neighbourhood. The composite task can be allocated to $\varAgent{}{}$ but cannot be successfully completed.
		}
	\end{enumerate}
\end{property}
\begin{property}[Optimal joint allocation in disjoint neighbourhoods]
	If all sets of neighbourhoods in 
	a system are pairwise disjoint then the optimal joint allocation is the union of all system optimal allocations.
	\begin{align}	
		\functionNeighbourhoodSignature{\varAgent{1}{}}{} &
		\cap \functionNeighbourhoodSignature{\varAgent{2}{}}{}
		= \emptyset, \forall (\varAgent{1}{}, \varAgent{2}{}) \in (\setAgent{}{} \times \setAgent{}{})\text{ where } \varAgent{1}{} \not = \varAgent{2}{}\nonumber \\
		& \implies 
		\setOptimalJointSystemAllocation{}{}
		\funcdef
		\bigcup
		\functionSystemOptimalAllocationSignature{}{}
	\end{align}
\end{property}

\begin{property}[Resource contention in non-disjoint neighbourhoods]
	If not all neighbourhoods in 
	the system are pairwise disjoint then there can be resource contention on the agents in the intersection of the neighbourhoods. If the impact of resource contention on allocation quality is sufficient, then the optimal joint allocation may no longer be the union of all system optimal allocations. In this case the optimal joint allocation of tasks cannot be decomposed and solved independently and must be solved centrally, or through agent coordination, greatly increasing the complexity of the solution. 
\end{property}


==> review.tex <==
\section{Review}
\todo[inline]{DELETE ON COMPLETION}

\subsection{Validated Points}

\subsubsection*{Major}

\begin{enumerate}
	\item The background citations are not specific or recent enough.
	XXXX
	\item The relevance to practical situations is not clear.
	XXXX
\end{enumerate}

\subsubsection*{Minor}
\begin{enumerate}
	\item XXXX
\end{enumerate}

\subsection{Reviewer: 1}

Recommendation: Major Revision

Comments:
This paper presents:
- combination of 4 algorithms that leads to MARL for decentralized task allocation
- an review of the domain which is quite general (maybe too general) and maybe a bit outdated. Everything seems at least 5 year old.
- a formalization of the DTAS problem
- a formalization of the proposed solution
- experiments to validate the approach

As I said, my MAJOR problem comes from the fact that I could not understand large and essential parts of the paper. I will try to explicit that below and try to offer some hints to improve the presentation, but I do not think I will be able to pinpoint every problem of the paper as some seem not significant until the main ideas are not correctly presented.

The overall structure and the writing of the paper are quite clear.

** Section 2
From you general State of the Art, it is not clear, concretely, what existing elements of the literature will help you build your proposition. It remains very general.

** Section 3

I had some problem reading and understanding many aspects of this section.

First, I would suggest you use 3 different kind of notations to differentiate objects. In particular I have been annoyed by $AT$ which seems to be a the space of sets or a particular set, depending on the equations or paragraph it is used.

spaces (for example use ${\mathcal A}$ for spaces of Sets

* set could be notated in capitals (like $AT$)

* an atomic object in small-case (like $at$)

=> In particular, for $AT$. Definition 3.1 cite AT as a set of atomic tasks. But then, section 3.3.1, I have some problem with a sentence like "IF $AT$ represents all the current atomic tasks in the system then...". So, the AT of section 3.3.1 can be a subset of the AT of 3.1 ?

Then, many notations use have some sort of incoherence :
=> Def 3.1 : an agent $g$ is defined by $<c,r,\delta_n,\delta_k>$. In definition 3.2, $g=<c,\delta_n,\delta_k$ (where is $r$ ?)
=> Sec 3.3.1, sorry but $|al(AT,g)|$ is NOT a set, it is, at best, the cardinally of a set yet to be defined.
=> paragraph before Def 3.3. An "atomic" allocation $<{at},t,g,a>$ has $a$ as the agent performing the task. Later, same paragraph, the set $L$ is made by tuples $<T,t,g,a>$ and this time, $a$ is the agent that allocatED the task.

Example 3.4 is nice.

My biggest problem is understanding how you consider allocation and the quality (and thus optimallity) of an allocation. Given a set of tasks $AT$ and a group of agent $AG$, there could be *several* allocations, and al(AT,G) is only *one* on these possible allocations. OK ? (But this could explicitly said somewhere).

I strongly think that explicit specifying the $al$ in the quality function $ql()$ would clarify this point. Right now, the dependence on a particular $al$ in implicit and hidden in equation (1). 
Then, in equation (2), some atomic tasks are completed. What is the explicit link between theses atomic tasks and the $i$ index ? Is the $at_i$ part of the $AT$ of $ql_i$. Is $AT$ constant ? Why ??? Same for G ??

Same for $ol*$ in equation (3). 

Equ(7) why the $g$ and $at$ of $ql( al(at,g) )$ are not between {} to be coherent and refer to sets ? Besides, this optimal joint system allocation only consider atomic allocations ? (And, formally, $ql()$ need 3 arguments, not 2....)

Overall, at the end of section 3.3.2 I really failed to see and understand the differences between all these qualities and best allocations. I am confused and puzzled.
I REQUIRES clarification, and AT LEAST, an clear and complete example.

Saying Theorem 3.10-3.12 are theorems is maybe too much? A property, maybe.


Besides, later (equation 13), you use $ql*$ which is not defined anywhere. Could it be $ol*$ instead. ?

[Side problem, but important] What it the rational behind using the number of concurrent allocation is assessing the quality of an allocation ? This is neither explained nor discussed anywhere, just defined.

** Section 4

Here I am mostly puzzled by your use of the Reinforcement Learning, both in term of Framework and in term of algorithm.

The way you use the RL concept is original (right now, I cannot say if it's right or wrong) and you should explicit your differences with the "classical" setting. In particular, the QValue you use is far from classic. It makes this section hard to understand.

With you definition of the QValue as a tuple $(action, likelihood of optimality)$, I fail to see how "Temporal difference update" (which you should call otherwise) can update this *tuple* (eq 12). Maybe it does only update the $likelihood$ part of the Q tuple ? Even in that case, what your QValue will converge to is clearly uncertain and impossible to predict as classical RL algorithm like the real TD update require some hypothesis to have a meaning:
- QValue must be linked to a *markovian state*. I think I understand that state (which you call "configuration" in section 3 and "state" in section 4) is given by your $qm(G,AP)$ function. But this far from being the "state" of the system, at best it is a partial view of the system. And, classical RL suggests/show that TD will not converge to anything meaningful (in general). So, if you do get some meaningful results, it should be emphasized and discussed and explained.

About 5.3 "Predicting the effect of actions"

In a classical RL setting, this should not be needed ? Why is it needed here. What part of your RL implementation is weakened and requires adding this effect prediction for you system to work ?
You try to formalize this "effect" (using sometimes unknown or new notations) to eventually explain you will have to estimate this probabilities. And, again, your hypothesis (importance of being at the intersection of J and K,) is not explained or discussed, just defined and used.
Definition 5.5 is really a definition ?

About TSQM. I totally failed to understand and apprehend the concept !
(Beside, I think you speak about this TQSM and its concept a bit sooner than in section 5.5.1. Maybe introduced in 5.5 ?) And section 5.5.2 is impossible to understand (for me at last). It makes no sense.

** 6 Evaluation

Apart from saying that I appreciate the idea of testing the several "units" or modules of your algorithm, I cannot say much because I do not understand the concepts (quality, RL, TQSM) behind your work.

I have the feeling that your experiments are nicely executed. This said, I am surprised because it seems you only make 1 run of each (potentially stochastic) experience. You should have several runs and presents some statistics (variance, mean, best, worse) about them. Or make it clearer that you have run several time each experience. Maybe this is hidden behind the term "episode" ?

I do not know if it is possible, but some sort of comparison with related work or related results would be nice (but, again, I do not know if it is possible or pertinent).


Additional Questions:
Review's recommendation for paper type: Full length technical paper

Should this paper be considered for a best paper award?: No

Does the paper present innovative ideas or material?: Yes

In what ways does this paper advance the field?: Up to my knowledge and understanding of this paper, ideas presented seem original and tackle pertinent and open problem in the field of MAS and task allocation.

In particular, I appreciated what seems to be a kind of intrinsic self-motivation through reinforcement where individual agent try to locally improve their average performance, relying on local information.

BUT, the biggest problem, as detailed below, I could not really understand all the methodology proposed by the paper...

Is the information in the paper sound, factual, and accurate?: No

If not, please explain why.: The "No" has several explanation, the main one being that I could not get a clear understanding of the methodology and ideas behing the paper proposed algorithms (I WILL detail below). So I am not able to correctly assess if information is "sound". Besides, regarding the way some aspect of Reinforcement Learning is presented, it is a bit too much uncommon (and somehow "twisted" without explicit warning) that I can not qualify this part of "accurate".

Finally, I have not been totally convinced by some details (notations and its coherence) of the problem and solution formalization.

Rate the paper on its contribution to the body of knowledge to this field (none=1, very important=5): 3

Rate how well the ideas are presented (very difficult to understand=1 very easy to understand =5): 1

Rate the overall quality of the writing (very poor=1, excellent=5): 4

Does this paper cite and use appropriate references?: Yes

If not, what important references are missing?: But I miss a bit some comparison with related ideas and applications. Conceptual references are mostly at least 5 years old and, without being an expert of the field, I would suppose there might have been some newer contributions that needs citing.
Besides, the only two 2020 references are not even complete (only authors and title !). Could not really see what their message is. And some other references are not correct either.

Should anything be deleted from or condensed in the paper?: No

If so, please explain.: But MAJOR rewriting is in order.

Is the treatment of the subject complete?: No

If not, What important details / ideas/ analyses are missing?: As said (and detailed later), I miss some information (maybe example and explanations) to really understand the paper.

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: Heavy

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: Maybe

\subsection{Reviewer: 2}

\subsubsection*{Recommendation:}
Major Revision

\subsubsection*{Comments:}

The paper tackles the problem of distributed task allocation using multi-agent reinforcement learning-based techniques. Overall the paper is (very) well written, targets a wide scope of problem that are relevant and important to the MARL community, provide extensive description of the techniques used (4 algorithms that are combined together in a framework called ATA-RIA) and a well-built evaluation (that compare how different setups of the multi-agent approach perform against an optimal solution in a simulated environment). All these reason tend to confirm the work undertaken is relevant for TAAS and that the approaches presented show strong interest. The evaluation shows interesting results (for instance on system resilience and on the impact of the number of agents involved) and some scenarios (for instance disabling some components of the framework) are really interesting to show how each algorithm contributes to the final results.

There are two major points that would require attention in the paper:

\begin{enumerate}
\item The current version of the paper lacks in justification and positioning with regard to existing work. This would strongly reinforce the paper’s contribution and give a better (and more fair/accurate) view of the extent of the work. Related work section introduces the various (but known) problems of MARL systems quite well, pointing out important challenges the research community has been investigating extensively. However, this section needs more discussion on how existing techniques address all the problem stated. For instance, the paragraph about large state-action spaces exploration suggest the problem is new and not addressed in the literature, while there are numerous approaches (like state-space adaptation, aggregation, generation, etc.) that specifically target it. It is not clear why more agents implies a greater dimensionality of the system, why would each agent state-space grow? Etc. Similarly, the exploration/exploitation tradeoff is central for the RL community and the section would benefit from discussing the limits of state-of-the-art approaches tackling this issue. The rest of the section also tend to make the reader into thinking all the problems remains not addressed (even in part) and this does not help to evaluate (or compare) the contribution brought by the approaches presented in the paper or to understand how the paper positions relatively to existing work. The novelty of each algorithm (independently) is also barely mentioned while their combination seems completely new. The presentation of the multi-agent task allocation system problem and model is clear and look consistent, although it is hard to know if this is a novel formalization or not, a new problem or not, etc. Similarly, the presentation of algorithms is exhaustive and well written, but very few links to existing work is made (except for the Temporal Difference update),  suggesting everything is novel while there must be bits of inspiration taken from related work (otherwise, it would be essential to better highlight the level of novelty and more than critical to justify the choices made within each algorithm). Evaluation section contains variations of the approach that are compared to the optimal solution. The paper would really benefit from adding either a strong justification on how existing work does not fit the stated problem or instead showing the difference between ATA-RIA algorithm and similar work.

\item The problem stated is presented from a quite generic and high-level perspective, and so is the simulated environment used for evaluation. Thus, the problem statement/simulated environment seems a bit far from practical applications. The paper would greatly benefit from providing a concrete and detailed example of such an environment or from discussing how the proposed framework can be used in a more realistic setup. A few domains are discussed in conclusion but the reader might expect a more detailed and realistic problem that would better show the potential of applying the framework presented.
\end{enumerate}
	
\subsubsection*{Additional minor questions:}

\begin{enumerate}
\item is the performance capped when the number of agents continues to increase? what explains that there seems to be a local optimum setup in the results for <large system> simulations?
\item could the authors further explain the gap observed in performance for the volatile system scenario with SAS-KR and RT-ARP enabled/disabled? could further research improve them? How are these two elements of the framework important for other scenarios?
\end{enumerate}

\subsubsection*{Summary}

Review's recommendation for paper type: Full length technical paper

Should this paper be considered for a best paper award?: No

Does the paper present innovative ideas or material?: Yes

In what ways does this paper advance the field?: The paper introduces 4 algorithms that cover different aspects of the distributed task allocation problem. It also presents and evaluates a framework that combine all components in different multi-agent RL setups. Each component targets a specific problem that remains of interest for the MARL community.

Is the information in the paper sound, factual, and accurate?: Yes

If not, please explain why.: 

Rate the paper on its contribution to the body of knowledge to this field (none=1, very important=5): 4

Rate how well the ideas are presented (very difficult to understand=1 very easy to understand =5): 3

Rate the overall quality of the writing (very poor=1, excellent=5): 5

Does this paper cite and use appropriate references?: No

If not, what important references are missing?: Cited references are relevant and adequate, however the related work section misses to mention important (and more recent) work on domains like state-space adaptation, exploration/exploitation dilemma, reward assignment models, multi- agent coordination, etc. that are well introduced as part of the scope of the paper.

Should anything be deleted from or condensed in the paper?: No

If so, please explain.: 

Is the treatment of the subject complete?: No

If not, What important details / ideas/ analyses are missing?: This point appears really difficult to assess, since the scope of the problem tackled in the paper seems really wide and algorithms presented target sub-parts of the problem with very few guarantee that they do combine to treat the problem fully. However, the objectives of the work are clearly stated, and seem reasonable, while being a bit less ambitious than the problem stated (points 1-4 in page 4).

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: Light

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: Maybe




==> shared.tex <==
\setboolean{draft}{false}

%TODO: Journal metadata
% Metadata Information
\acmJournal{TAAS}
\acmVolume{0}
\acmNumber{0}
\acmArticle{0}
\acmYear{2021}
\acmMonth{0}
\copyrightyear{2021}
%\acmArticleSeq{9}

% Copyrightbrew update
\setcopyright{acmlicensed}

% TODO: DOI
% DOI
\acmDOI{0000001.0000001}

%TODO: Paper history
% Paper history
%\received{February 2007}
%\received[revised]{March 2009}
%\received[accepted]{June 2009}

% DEFINE THE PAPER TITLES
\newcommand{\chapterOptimalNeighbourhoods}{\chapter{Dynamic neighbourhood optimisation for task allocation using multiagent learning}}
% DEFINE THE PAPER TITLES
\newcommand{\sectionOptimalNeighbourhoods}{\section{Dynamic neighbourhood optimisation for task allocation using multiagent learning}}


% Document starts

\begin{document}
% Title portion. Note the short title for running heads
\title{Dynamic neighbourhood optimisation for task allocation using multiagent
learning}
\maketitle

%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below.
%
\begin{CCSXML}
	<ccs2012>
	<concept>
	<concept_id>10003752.10010070.10010071.10010261.10010275</concept_id>
	<concept_desc>Theory of computation~Multi-agent reinforcement learning</concept_desc>
	<concept_significance>500</concept_significance>
	</concept>
	<concept>
	<concept_id>10010147.10010178.10010219.10010220</concept_id>
	<concept_desc>Computing methodologies~Multi-agent systems</concept_desc>
	<concept_significance>300</concept_significance>
	</concept>
	<concept>
	<concept_id>10010147.10010178.10010219.10010221</concept_id>
	<concept_desc>Computing methodologies~Intelligent agents</concept_desc>
	<concept_significance>300</concept_significance>
	</concept>
	<concept>
	<concept_id>10010147.10010178.10010219.10010223</concept_id>
	<concept_desc>Computing methodologies~Cooperation and coordination</concept_desc>
	<concept_significance>300</concept_significance>
	</concept>
	<concept>
	<concept_id>10010520.10010521.10010537.10010540</concept_id>
	<concept_desc>Computer systems organization~Peer-to-peer architectures</concept_desc>
	<concept_significance>100</concept_significance>
	</concept>
	<concept>
	<concept_id>10010520.10010553.10003238</concept_id>
	<concept_desc>Computer systems organization~Sensor networks</concept_desc>
	<concept_significance>100</concept_significance>
	</concept>
	</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Theory of computation~Multi-agent reinforcement learning}
\ccsdesc[300]{Computing methodologies~Multi-agent systems}
\ccsdesc[300]{Computing methodologies~Intelligent agents}
\ccsdesc[300]{Computing methodologies~Cooperation and coordination}
\ccsdesc[100]{Computer systems organization~Peer-to-peer architectures}
\ccsdesc[100]{Computer systems organization~Sensor networks}

%
% End generated code
%

% TODO: Keywords
\keywords{Wireless sensor networks, media access control,
multi-channel, radio interference, time synchronization}

% The default list of authors is too long for headers.
\renewcommand{\shortauthors}{N. Creech et al.}
\raggedbottom
\ifbool{overwrite-includes}
{}
{
	\input{common_definitions}
	\input{acm_introduction}
	\FloatBarrier
	
	\input{abstract}
	\FloatBarrier
	\input{introduction}
	\FloatBarrier
	\input{background}
	%\input{background-extended}
	\FloatBarrier
	
	% PROBLEM SECTION 
	\ifbool{extended}{
		\input{problem_definition-extended}
		\FloatBarrier
	}{}
	\input{problem}
	\input{problem-allocation-optimality}
%	\input{problem-examples}
	\input{problem-statement}
	%\input{problem_definition}
	%\input{problem-tasks}
	%\input{problem-neighbourhoods}
	%\input{problem-allocations}
	%\input{problem-quality}
	%\ifbool{extended}{
	%	\input{problem-system_space}
	%}{}
	%\input{problem-optimal_allocations}
	%\input{problem-task_allocation_problem}
	% ALGORITHMS SECTION
	\input{algorithms-summary}
	\FloatBarrier
	% SOLUTION SECTION 
	\ifbool{extended}{
		\input{solution-extended}
		\FloatBarrier
	}{}
	\input{solution}
	%\input{solution-action_types}
	%\input{solution-action_instances}
	%\input{solution-action_samples}
	%\input{solution-neighbourhood_quality}
	\input{solution-action_probabilities}
	\input{solution-reinforcement_learning}
	\ifbool{extended}{
	\input{solution-state_action_space}
	}{}
	\input{prediction}
	\input{prediction-impact_on_neighbourhood}
	\input{prediction-action_impact}
	\input{prediction-historical}
	\FloatBarrier
	\input{algorithms}
	\FloatBarrier
	
	% Simulation
	\ifbool{extended}{
		\input{simulation-extended}
		\FloatBarrier
	}{}
	\input{simulation}
	
	% RESULTS
	\FloatBarrier
	
		\ifbool{extended}{
		\input{results-extended}
		\FloatBarrier
	}{}
	\input{experimental}
	\input{results}
	\input{results-task-allocation}
	\input{results-exploration}
	\input{results-resilience}
	\input{results-graphs}
	\FloatBarrier

	\input{conclusions}
	\FloatBarrier
	\input{references}
	\FloatBarrier
\begin{appendices}
		\input{symbols}
		\FloatBarrier
		%\input{algorithms-flow}
		\FloatBarrier
		\input{tables}
		\FloatBarrier
		\input{tables_results}
		\input{algorithms-standard}
		\FloatBarrier
	\ifbool{debug}{
		\include{revisions}
		\FloatBarrier
		\input{appendices}
		\FloatBarrier
	}{}
\end{appendices}
	}
\ifbool{overwrite-includes}
{}
{\end{document}}




==> solution-available-states.tex <==
\subsubsection{Q-values}
As previously mentioned in Definitions \ref{def:agent-state} and \ref{def:system-state}, the system state can be specified as $\setState{}{} = \langle \setAgent{S}{}, \setJointSystemAllocation{}{} \rangle$, where the set of agent states $\setAgent{S}{}$ are defined by the knowledge and neighbourhood of each agent, $\langle  K, N \rangle$. For each state there exists \textit{Q-value} tuples, $\varQ{}{} \funcdef \tupleQ{}{},  \varQProb{}{} \in \setRealNumbersUnit{}{}$, where $\varQProb{}{}$ is the \textit{action-likelihood} that $\varAction{}{}$ is the optimal action to perform in the the given state. Q-values are mapped to each agent and atomic task  type, $\formalQMapping{}{}$. {This mapping forms the agents' policy.}

\subsubsection{The availability of actions}
Not all of the actions an agent knows of are available for it to take. For example an agent $\varAgent{}{}$ cannot perform an allocation action $\text{ALLOC}(g, at, n)$ if $n \in \functionKnowledgeSignature{}{}$ but $n \not \in \functionNeighbourhoodSignature{}{}$. We refer to these \textit{unavailable actions} $\setUnavailableActions{\varAgent{}{}}{}$ as actions that involve agents in an agents' knowledge base, but are not currently in its neighbourhood. An agents' set of \textit{available actions} $\setAvailableActions{\varAgent{}{}}{}$ are the actions it can take given its unallocated atomic tasks, neighbourhood, and knowledge. We can then additionally define $\setAvailableQ{}{}$ and $\setUnavailableQ{}{}$ as available and unavailable Q-values respectively, those values that refer to available or unavailable actions. 

==> symbols.tex <==
\section{Mathematical notation}
\begin{table}[H]
\centering
\captionsetup{labelfont=bf,singlelinecheck=on,justification=raggedright}
\caption{Summary of task symbols}
\label{table:summary_of_task_symbols}
\begin{tabular}{|p{0.2\textwidth}|p{0.2\textwidth}|p{0.5\textwidth}| }
\hline
\multicolumn{3}{|l|}{\textbf{Tasks}} \\
\hline
$\varAtomicTaskType{}{}$ & Atomic task type & The type of an atomic task. \\
$\varCompositeTaskType{}{}$ & Composite task type & The type of a composite task. \\
$\varAtomicTask{}{}$ & Atomic task & An instantiation of an atomic task type. \\
$\varCompositeTask{}{}$ & Composite task & An instantiation of a composite task type. \\
$\varAgentCapability{}{}{}{}$ & Capability & The atomic task types an agent can complete. \\
$\varAgentResponsiblity{}{}{}{}$ & Responsibility & The composite task types an agent can oversee. \\
$\varAgentNeighbourhoodConstraint{}{}$ &  Neighbourhood constraint & Limit on the size of neighbourhood an agent can have.\\
$\varAgentKnowledgeConstraint{}{}$ &  Knowledge constraint & Limit on the amount of knowledge an agent can have. \\	
$\functionAtomicTaskMapping{}{}$ & Atomic task type mapping & Maps atomic tasks onto their corresponding atomic task types. \\
$\functionCompositeTaskMapping{}{}$ & Composite task type mapping & Maps composite tasks onto their corresponding composite task types. \\
$\functionAtomicTaskQualitySignature{}{}$ & Atomic task quality & Maps atomic task types, agents, and concurrent task count to quality values. \\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\captionsetup{labelfont=bf,singlelinecheck=on,justification=raggedright}
\caption{Summary of allocation symbols}
\label{table:summary_of_allocation_symbols}
\begin{tabular}{|p{0.15\textwidth}|p{0.2\textwidth}|p{0.6\textwidth}| }
\hline

\multicolumn{3}{|l|}{\textbf{Allocations}} \\
\hline
$\functionAtomicAllocationSignature{}{}$ & Atomic task allocation & Maps a set of atomic tasks to a subset of system agents. \\
$\functionQLSignature{}{}$ & Allocation quality & The quality obtained by allocating tasks $\setAtomicTask{}{}$ to agents $\setAgent{}{}$ when there is a joint system allocation $\setJointSystemAllocation{}{}$  \\
$\functionSystemUtility{}{}$&  System utility & The sum of the allocation qualities obtained over a time period $\setTime{}{}$ \\
$\setAtomicTaskUnallocated{}{}$ & Unallocated atomic tasks & The set of atomic tasks that have not been allocated to child agents. \\
$\functionLocalOptimalAllocationSignature{loc}{}$ & Locally optimal allocation & The atomic task allocation that maximises the quality of an agents composite task. \\
$\functionOptimalNeighbourhoodSignature{}{}$ & Optimal neighbourhood & The neighbourhood containing the agents required to obtain the highest value locally optimal allocation. \\
$\functionSystemOptimalAllocationSignature{}{}$ & System-optimal allocation & The locally optimal allocation to the optimal neighbourhood. \\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\captionsetup{labelfont=bf,singlelinecheck=on,justification=raggedright}
\caption{Summary of action symbols}
\label{table:summary_of_action_symbols}
\begin{tabular}	{|p{0.15\textwidth}|p{0.2\textwidth}|p{0.55\textwidth}| }
\hline
\multicolumn{3}{|l|}{\textbf{Actions}} \\
\hline
$\setAvailableActions{\varAgent{}{}}{}$ & Available actions & The possible actions an agent can take given its current state\\
$\setNeighbourhoodTargetActions{}{}{}$ & Child target actions & The set of actions where child agents in the set $\setAgent{}{}$ are targets of the parent agent $\varAgent{}{}$\\
\hline
\multicolumn{3}{|l|}{\textbf{Action sampling}} \\
\hline
$\setActionSample{}{}$ & Action samples & A set of records of actions taken\\
$\functionActionSampleSelectorSignature{}{}$ & Action sample selection function & Function to select subsets of action samples\\

$\varSampleTime{}{}$ & Sample time & The time an actions was taken \\
$\varSampleValue{}{}$ & Sample value &  The quality value when an action was taken\\ 
$\setAgentActionSamples{}{}$ & Agent action sample & The set of all action samples for a specific agent\\
$\functionLastActionSampleSignature{}{}$ & Last action sample & The action sample with the latest sample time\\
$\functionUncertainInformationSignature{}{}$ & \acronymActionInformationQuality{UPPER}{} & The value of an agents information of an action obtained through sampling \\
$\varUncertainInformationThreshold{}{}{}{}$ & Information retention threshold & A system constant that sets the level at which action knowledge is considered discardable\\
$\functionMQNSignature{}{}$ & Minimum quality neighbour & The agent whose action samples within the set $\setAgentActionSamples{}{}$ produced the lowest sum of quality values.\\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\captionsetup{labelfont=bf,singlelinecheck=on,justification=raggedright}
\caption	{Summary of Q-space symbols}
\label{table:summary_of_q_space_symbols}
\begin{tabular}	{|p{0.2\textwidth}|p{0.2\textwidth}|p{0.50\textwidth}| }
\hline
\multicolumn{3}{|l|}{\textbf{Q-space}} \\
\hline
$\setQ{}{}$ & Q-values & $(\varAction{}{}, \varQ{}{})$ tuples where $\varQ{}{}$ is the likelihood that taking an action $\varAction{}{}$ in an agents' current states is optimal\\
$\setAvailableQ{}{}$ & Available Q-values & Q-values with actions that are able to be taken by agents in their current states\\
$\setAvailableQ{}{}$ & Unavailable Q-values & Q-values with actions that cannot be taken by agents in their current states\\
$\functionQMappingSignature{}{}{}$ & Q-mapping & Maps an agent and task types to Q-values\\
$\functionOLMetricLocalSignature{}{}$ & Locally optimal allocation metric & The difference
between an allocations quality and the locally optimal quality possible for that allocation\\
$\functionOLMetricSystemSignature{}{}$ & System optimal allocation metric & The difference
between an allocations quality and the system optimal quality possible for that allocation\\
$\functionNISignature{1}{2}$ & Neighbourhood impact & The difference between two neighbourhoods optimal composite quality values\\
$\functionKISignature{}{}$ & Knowledge impact & The difference between the possible optimal composite quality values that can be formed from neighbourhoods within two knowledge bases \\
$\setRewardSet{}{}$ & Time-summarised quality matrix (TSQM) & The ordered set of past quality values of an agent, summarised by row\\
$\functionImpactInterpolationSignature{}{}$ & Impact interpolation function & A linear interpolation over the rows of a TSQM\\
$\functionImpactTransformationSignature{}{}$ & Impact transformation function & A probability estimate that taking an action-type in the current neighbourhood will generate better future quality values \\
\hline
\end{tabular}
\end{table}

